Unsupervised Meta-Learning through Latent-Space Interpolation in Generative Models

Unsupervised meta-learning approaches rely on synthetic meta-tasks that are created using techniques such as random selection, clustering and/or augmentation. Unfortunately, clustering and augmentation are domain-dependent, and thus they require either manual tweaking or expensive learning. In this work, we describe an approach that generates meta-tasks using generative models. A critical component is a novel approach of sampling from the latent space that generates objects grouped into synthetic classes forming the training and validation data of a meta-task. We find that the proposed approach, LAtent Space Interpolation Unsupervised Meta-learning (LASIUM), outperforms or is competitive with current unsupervised learning baselines on few-shot classification tasks on the most widely used benchmark datasets. In addition, the approach promises to be applicable without manual tweaking over a wider range of domains than previous approaches.

==> sections/BroaderImpact.tex <==
\section*{Broader Impact}

The contributions of this paper expand the accuracy and applicability of few shot learning into domains where there is a limited amount of labeled data available. The practical impact of these results is that (a) users who cannot afford extensive data collection and labeling campaigns can develop competitive classifiers and (b) better performance can be obtained in classification applications where the amount of labeled data is naturally low. 

There are many ways these advances can be put to a positive societal use. For instance, the approach can be used to classify medical images for rare illnesses, or illnesses where insufficient training data is available. Interestingly, COVID-19 at the time of the submission of this paper falls into this category in the United States. As part of our ongoing work to apply our research to practical applications, we found that as of June 2020, the COVIDx dataset~\cite{wang2020covid} is currently the largest accessible repository of COVID imaging in the US. This dataset contains 76 radiography images from 53 COVID-19 patient cases. Despite the prevalence of the illness, classifying these by severity maps them exactly into the few shot learning scenarios considered in this paper. 

Naturally, any AI image classification technology can be put to negative use, for instance by repressive regimes improving their surveillance systems. 

%AI quickens its pace to be similar to humans and beats humans in many fields. A few examples include AlphaGo~\cite{ alphago2016} beated human champions in the ancient game of Go, besides, residual network (ResNet)~\cite{ResNet2016} achieved better classification accuracy performance than humans on ImageNet dataset. AI also supports the development of intelligent tools in many aspects of daily life, such as voice assistants, search engines, autonomous driving cars, and industrial robots. In spite of its progress, current AI techniques hampered to generalize from limited amount of available data. The aforementioned prosperity of AI applications is contingent upon learning from data-intensive cases. This is while, in practice due to the privacy, safety or ethic issues we do not have access to a large number of data. In contrast, humans are able to learn new tasks quickly by taking into account what they learned in the past. For instance, given a few photos of a stranger, a child can easily identify the same person from a large number of photos verifying the ability of learning new concepts and the generalization after just a few examples of a given object.

%Decreasing this gap between AI and humans’ performance is an important research field which can be tackled by Meta-Learning. Meta-Learning can be a tool for societal progress. Think of robotics~\cite{robotics-book2009}, which develops machines that can replicate human actions which in turn improves the lives of people with disabilities. This research paper can tackles some societal challenges such as drug discovery~\cite{drugdiscovery-2017} as well. Because of potential toxicity, and low activity, new molecules do not have enough real biological records on clinical candidates.  Classification of medical images for rare illnesses, or illnesses where insufficient training data is available is the other application of meta-learning where the society can benefits from. Surprisingly, at the time of the submission of this paper COVID-19 is around. We found that as of June 2020, the COVIDx dataset~\cite{wang2020covid} which is currently the largest accessible repository of COVID imaging in the US, still contains 76 radiography images from 53 COVID-19 patient cases which is a small amount of data. Therefore, our proposed algorithms can contribute in this regime of limited data in order to classifying the images for the severity maps. All in all, it is important to learn effectively from a small number of samples. Here in this work, leveraging the advantages of generative models such as GANs and VAEs, we generate new pairs of in-class and out-of-class data for the meta-learning process. This process is being done with the help of our proposed algorithm, LASIUM. Finally, it worth mentioning that the impacts of this research project extend beyond the borders of an institution or country. Lives can be shaped for the better with the result of this work.




==> sections/NotIncluded.tex <==

% such as MSGAN (Miss-GAN)~\cite{mode-gan-Qi2019} and progressive growing of GANs~\cite{karras2017progressive} as well as standard variational autoencoder (VAE)~\cite{kingma2013auto} to generate in-class and out-of-class pairs of meta-training data. 



% tend to outperform approaches based on transfer learning or other unsupervised pre-training approaches, but 


% Relatively few works have analyzed the unsupervised meta-learning. Only very recently, researchers have proceeded to develop unsupervised few-shot learning algorithms. 
% A recent and promising algorithm, namely CACTUs studied in~\cite{hsu2018unsupervised}, where a progressive clustering method is used to leverage feature representations before doing task training. 
% Hsu et al.~\cite{hsu2018unsupervised} proposed CACTUs that leverages feature representations before doing task training by using a progressive clustering method.
%Khodadadeh et al.~\cite{khodadadeh2019unsupervised} adopted a different perspective for unsupervised meta-learning. They proposed UMTRA algorithm that utilizes the statistical diversity properties and domain-specific augmentations to generate training and validation data in the meta-learning procedure.
% A different perspective adopted in~\cite{khodadadeh2019unsupervised} for unsupervised meta-learning in which the UMTRA algorithm was proposed. 
% Antoniou and Storkey~\cite{AAL2019} proposed AAL which employs data augmentations of the unlabeled training set to generate the validation data. 

% The main idea of these papers is that we can leverage unsupervised embedding to construct tasks for a meta-learning algorithm. 

% This leads us to the LASIUM algorithm that is particularly effective as it is versatile for generating in-class and out-of-class pairs of data for meta-learning as well as is not domain-specific. 
% To the best of our knowledge, none of these prior work studied the proposed scenario of this work.
% ~\cite{huangfewshot2019} proposed a method for unsupervised few shot learning which leverages performing clustering without labels during the meta-evaluation time. It further proposes a Centroid Networks to measure hardness of building tasks when the class semantics vary across different tasks.




% {\bf{Learning-based Data Augmentation (DA)}}
% {\bf{Deep generative models}}
% The generative adversarial network (GAN)~\cite{goodfellow2014generative} and variational autoencoder (VAE)~\cite{kingma2013auto} have achieved significant success in many unsupervised learning problems. 


% Generative models have been explored for semi-supervised learning and have achieved significant improvements.

% We develop a learning-to-learn process to optimize the proposed feature-wise transformation layers for ....

%Our model chooses a similar approach to train the proposed feature-wise ..., however, differs from prior work as we focus on ...

%In meta-Learning rather than emulating Bayesian inference, models are trained end-to-end in order to accomplish a learning task by building classifiers from a few training examples.

%{\bf{Domain generalization}}
%Domain generalization and transformation have been attracting steady increase of interests in deep learning community in the last few years\cite{Blanchard2011}. It has achieved impressive performance due to recent development of GANs~\cite{kim2017-domain}. Domain generalization methods tends to generalize from a set of seen domains to the unseen domain without having access to the instances from the unseen domain during the training process. Prior to the advent of
%the meta-learning approaches, several frameworks have been suggested in order to tackle the domain generalization problem. For example, \cite{Blanchard2011, Li-cvpr2018} focused on extracting domain-invariant features from various seen domains. \cite{Niu-cvpr2015} proposed a model to ameliorate the classifiers via fusing classifiers learned from seen domains. Another line of work presented in~\cite{Li-iccv2017} decomposes the classifiers into domain-specific and domain-invariant components. Another stream of work learns to augment the input data with adversarial learning~\cite{Volpi2018, Shankar2018}.



% {\bf{Data augmenttion}}
% Data augmentation approaches are proposed to enhance the diversity of data for the training stage~\cite{Ekin-cvpr2018, Sixt2018, Perez2017, Tran-NIPS2017}.

% In particular, in~\cite{Tran-NIPS2017} a Bayesian DA method was proposed in which the data is augmented according to the distribution learned from the training set; RenderGAN model in~\cite{Sixt2018} simulates realistic images making use of GANs; AutoAugment algorithm~\cite{Ekin-cvpr2018} does the augmentation via reinforcement learning (RL);~\cite{Shankar2018,Volpi2018} proposes frameworks for augmentation of the data by modeling to the variation across various domains with adversarial learning; and finally,~\cite{khodadadeh2019unsupervised} exploits the statistical diversity of the data and domain-specific augmentations to build tasks in the meta-learning procedure. 




% Method

% In this section we describe the method for our algorithm. What we want to achieve is semi supervised meta-learning.  UMTRA~\cite{khodadadeh2018unsupervised} achieves this by augmentation without any labeled information. CACTUs~\cite{hsu2018unsupervised} achieves this by clustering the data with unsupervised features and generating tasks based on clusters. In this paper, we study the spectrum from unsupervised meta-learning to supervised meta-learning by applying active learning to select data points. Active learning techniques allow us to choose data points which are more informative. Then you can ask an oracle to label these data points for you and use their supervision signal. One challenge here is that, we want to generate tasks from labelled data and unlabeled data points and just picking data points which are labeled by themselves does not enable us to make tasks automatically. For example consider the case when we choose 1000 data points and label them and only one of them belongs to the class Cats. How can we generate tasks from this class?
% \begin{itemize}
%     \item Pick some data points which are more informative
%     \begin{itemize}
%         \item Use iterative projection~\cite{zaeemzadeh2019iterative} (Problem is that this one itself requires feature space from imagenet)
%         \item Use GANs~\cite{sinha2019variational}
        
%     \end{itemize}
%     \item train a network based on these points
%     \item Learn a feature space for all data points.
%     \item Map all data points to this feature space. (implemented)
%     \item use these feature space and a metric distance to generate tasks (implemented)
%     \item apply meta-learning on these tasks (implemented)
% \end{itemize}

% 0.7572000622749329 +- 0.004985778250078231


%In this section, we provide required preliminaries and describe our approach for unsupervised meta-learning. 


% Concretely, we are dealing with an $N$-way, $(K^{(tr)}, K^{(val)})$-shot supervised learning task, $\Task$, that consists of two disjoint sets $\TaskTrain$ and $\TaskVal$.
% $\TaskTrain$, has exactly $i \in \{1, \ldots, N \times K^{(tr)}\}$ data points $(x_i, y_i)$ such that there are exactly $K^{(tr)}$ samples for each categorical label $y_i \in \{1, \ldots, N\}$. $\TaskVal$ contains another $N \times K^{(val)}$ data points separate from the ones in $\TaskTrain$. We have exactly $K^{(val)}$ samples for each class in $\TaskVal$ as well. 


% We propose a novel algorithm to generate tasks in an unsupervised manner by using generative models.

% we construct tasks from an unlabeled dataset $\mathcal{U} = \{x_{i}\}$. 
% A key challenge, then, is how to automatically build tasks from the unlabeled dataset $\mathcal{U}$. We propose a novel algorithm to generate tasks in an unsupervised manner by using generative models.


% In particular, to build an $N$-way classification task ${\cal{T}}$, we can sample $N$ classes, sample $K^{(tr)} + K^{(val)}$ instances from each class, and sample a permutation of $N$ distinct one-hot vectors to serve as task-specific labels of the $N$ sampled classes.

% Starting from an unlabeled dataset $\mathcal{U} = \{x_{i}\}$ drawn from an underlying distribution, $p(x)$, we are interested in learning a classifier $f$ that efficiently adapts and learns a probability distribution over the classes of new unseen human-specified downstream supervised learning tasks. 
% We assume these downstream tasks' inputs are different from the samples in $\mathcal{U}$ while drawn from the same distribution, $p$. This can appear as a semi-supervised learning problem. However, unlike semi-supervised learning, these tasks have different underlying class labels or attributes. Furthermore, we desire to learn these tasks with fewest training samples as possible, ideally one sample per class.
% We refer to the process of learning classifier $f$ from $\mathcal{U}$ that can adapt to any given task quickly as unsupervised meta-learning. 


% \subsubsection{Task definition}
% \label{TaskDefinition}
% Concretely, we are dealing with an $N$-way, $(K^{(tr)}, K^{(val)})$-shot supervised learning task, $\Task$, that consists of two disjoint sets $\TaskTrain$ and $\TaskVal$.
% $\TaskTrain$, has exactly $i \in \{1, \ldots, N \times K^{(tr)}\}$ data points $(x_i, y_i)$ such that there are exactly $K^{(tr)}$ samples for each categorical label $y_i \in \{1, \ldots, N\}$. $\TaskVal$ contains another $N \times K^{(val)}$ data points separate from the ones in $\TaskTrain$. We have exactly $K^{(val)}$ samples for each class in $\TaskVal$ as well. 

% \subsubsection{Meta-learning and task generalization error}
% The train and validation data for an $N$-way $(K^{(tr)}, K^{(val)})$-shot task, $\Task \in \{\mathcal{T}_{i}\}$, is drawn from an underlying joint distribution ${\cal{P^T_{X,Y}}}(x_i, y_i)$.
% Our goal is to learn a classifier $f_{\Task}$ to predict $y$ given $x$. In other words, $f_{\Task}(x) = {\rm{arg\,max}}_{y}{{\cal{P^T_{Y|X}}}(y|x)}$.
% % We do not have access to the underlying distribution ${\cal{P^T_{X,Y}}}(x, y)$, 
% We just have access to a few samples of the task train set, $\TaskTrain$. We can train a neural network, $f_{\TaskTrain}$, on the task train set.
% The estimate of the expected error on the task $\mathcal{T}$ is:
% % $\mathbb{E}_{(x_{i}, y_{i}) \in \TaskVal} {[(f_{\TaskTrain} - y_{i})^2]}$. 
% \begin{equation}
% {\cal{L}}_{{{\cal{T}}}}\left( {f_{{\cal{{D}}}^{(tr)}_{\cal{T}}}, \TaskVal } \right) = \sum\limits_{\left( {{x_i},{y_i}} \right) \in {\cal{{D}}}^{(val)}_{\cal{T}}} {{y_i}\log } f_{{\cal{{D}}}^{(tr)}_{\cal{T}}}\left( {{x_i}} \right) + \left( {1 - {y_i}} \right)\log \left( {1 - f_{{\cal{{D}}}^{(tr)}_{\cal{T}}}\left( {{x_i}} \right)} \right).    
% \end{equation}
% The average estimate of the expected error on a mini-batch of tasks drawn from $\{\Task_{i}\}$ is what we aim to minimize during meta-learning. Once the meta-learning algorithm is applied, we evaluate our meta-learned model on a set of tasks $\{\Task'_{i}\}$ which do not share any instance and even classes with the tasks from $\{\Task_{i}\}$ to evaluate the capability to adapt to new unseen tasks.


% \subsubsection{Unsupervised meta-learning}
% In the supervised meta-learning setting, given a labeled classification dataset $\mathcal{D}$ that comprises $M$ data points, $\{(x_{i}, y_{i})\}$, where $y_{i} \in \{1, \ldots, Q\}$ and $Q >> N$, it is straightforward to generate $N$-way, $\{K^{(tr)}, K^{(val)}\}$-shot tasks. In particular, to build an $N$-way classification task ${\cal{T}}$, we can sample $N$ classes, sample $K^{(tr)} + K^{(val)}$ instances from each class, and sample a permutation of $N$ distinct one-hot vectors to serve as task-specific labels of the $N$ sampled classes. Of course, the instances in $\TaskTrain$ and $\TaskVal$ are disjoint. Nonetheless, in the context of unsupervised meta-learning, a key challenge, then, is how to automatically build tasks from the unlabeled dataset $\mathcal{U}$. \cite{hsu2018unsupervised} introduced clustering to automatically construct tasks for unsupervised meta-learning (CACTUs). They cluster $\mathcal{U}$ via an unsupervised feature learning algorithm which maps every instance to a feature space, followed by applying K-means on the feature space. \cite{khodadadeh2019unsupervised} sample randomly from $\mathcal{U}$ and apply augmentation on the samples to maintain membership and generate different instances for different tasks. 
% We propose a novel algorithm to generate tasks in an unsupervised manner by using generative models. Not only, does our approach performs very well on the few-shot learning benchmarks, but also it is very general to use on different domains and requires minimum tweaking.
% We elaborate on these approaches in the following sections.




% Herein, in order to construct tasks in an unsupervised fashion that resembles that of the human-specified labels, we introduce some methods. 
% One of the methods is based on sampling vectors from a latent space representation designed for training an unconditional generative adversarial network (GAN)~\cite{goodfellow2014generative} trained on $\mathcal{U}$. The other method is based on\SV{now you can explain it here as you decided to add VAE according to your comment} .


% Generative models learn a probability distribution over the samples $x \in \mathcal{U} \sim p(x)$. We propose to leverage these models' capabilities to generate tasks for unsupervised meta-learning. In particular, we are more interested in generative model approaches that present a meaningful latent space. If we are able to generate samples similar to those in $\mathcal{U}$ which belong to the same class or even same visual cluster~\cite{hsu2018unsupervised} or have richly augmented~\cite{khodadadeh2019unsupervised, AAL2019}, we can generate useful unsupervised tasks. This reduces our problem to generating in-class and out-of-class pairs. In-class pairs are two vectors in latent space that their corresponding generated images belong to the same class. On the other hand, out-of-class pairs are two vectors in latent space that their corresponding generated images belong to different classes. Fig~\ref{fig:method-gan} and ~\ref{fig:method-vae} sketch the way that the tasks are built by GANs and VAEs.


% A common method to cope with limited amount of labels is DA~\cite{goodfellow2014generative}. Translation, noise, and other deformations can often be employed without changing the labels, thereby effectively increasing the number of training examples and reducing overfitting. 
% Adversarial training has received a wide range of applications in recent years, such as semi-supervised learning etc. However, the number of works have successfully combined adversarial training with few-shot learning is still sparse. 



% In-class pairs are two data points in the latent space of the generator that when we generate images from them, the generated images visually belong to the same class. Out-class pairs are two data points in the latent space of the generator that when we generate images from them, the generated images visually does not belong to the same class.
% Class border is not well defined. 
% We are sure that sticking around a point will remain in the same class (due to the way that we train our generative models).
% We are sure that in a latent space which is meaningful for interpolation the LASIUM-p2 and LASIUM-p3 generate in-class and out-class samples.
% We leverage generative modes to generate tasks for unsupervised meta-learning. 
% The fundamental idea of our approach is that in the latent space representation of a generative model in-class pairs should be close while out-of-class pairs are far.
% We build our approach based on the assumption that the latent embedding of the data in generative models is meaningful. In particular, the euclidean distance in the latent space is meaningful 

% Thus we can choose out-of-class pairs by choosing random objects from an unlabeled dataset and checking whether they are sufficiently far in the latent space representation. 
% We can generate in-class pairs by interpolating between two out-of-class samples in the latent space and choosing interpolation ratios that put the new sample close to one or the other objects. The generative model can generate the new in-class object. This approach requires minimal domain-specific tweaking, and the necessary tweaks are human-comprehensible. For instance, we need to choose thresholds for latent space distance that ensure that classes are in different domains, as well as interpolation ratio thresholds that ensure that the sample is in the same class as the nearest edge. Another advantage of the approach is that we can take advantage of off-the-shelf, pre-trained generative models. 


% Considering a GAN can implicitly learns a meaningful latent embedding of the data, we make use of an unconditional generative model to generate fake images that is close to the real ones in one specific task ${\cal{T}}$. Our approach begins with training an unconditional GAN on $\mathcal{U}$. A GAN consists of two main networks. A generator network $\mathcal{G}$, which takes $z$ as an input and generates an image $I$, and a discriminator network $\mathcal{d}$ which takes an image and classifies it as a real image if it comes from our dataset $\mathcal{U}$ or as a fake image if it generated by $\mathcal{G}$.


% The euclidean distance and direction are meaningful in the latent space of these models and this makes them a better choice for our method.
% We train the parameters of generator $\mathcal{G}$ and discriminator $d$ in a min-max game with the following objective function: $\mathop {\min }\limits_\mathcal{G} \mathop {\max }\limits_d V\left( {d,\mathcal{G}} \right) = {{\rm{E}}_{x \sim {p_{data}}\left( x \right)}}\left[ {\log d\left( x \right)} \right] + {{\rm{E}}_{z \sim {p_{data}}\left( z \right)}}\left[ {\log \left( {1 - d\left( {\mathcal{G}\left( x \right)} \right)} \right)} \right]$. 


% MSGAN adds another term to this loss $|z_i - z_j| / |\mathcal{G}(z_i) - \mathcal{G}(z_j)| $.
% We saw that adding this term will result in more variant images as well as a better latent space for our purpose. ProGAN as well have the interpolation ability between two images and is a suitable choice for us.


% Our generator $\mathcal{G}$ and discriminator $\mathcal{D}$  are implemented as multi-layer perceptron (MLP). 
% The random Gaussian noise $z \sim {\cal{N}}\left( {0,1} \right)$ and
% class embedding $y_i$ are concatenated and fed into the generator, which is composed of $XX$ fully connected layers with $XX$ hidden units. 
% We find dimension of noise XXXX, i.e. dimension of class embeddings, works well. Similarly, the
% discriminators take input as the concatenation of image feature and class embedding and have XXX fully connected layers with XXX hidden units. We use Leaky ReLU as the nonlinear activation function except for the output layer of G, for which Sigmoid....\SV{here we need to add some infos about the architetcure of our GAN model. I wrote some sample infos but would be good if Siavash you could update it as you implemented. Please read this paragraph. Or we can explain this in the experiment section}

% In order to construct an $N$-way $\{K^{(tr)}, K^{(val)}\}$-shot task, we need to generate $K^{(tr)} + K^{(val)}$ instances for each class.
% We apply an iterative procedure to construct a meta-task.
% We iteratively accomplish this goal by leveraging the features of the latent space representation. 


% For VAEs, we sample $N$ different data points from our dataset $\mathcal{U}$ and encode them into $N$ vectors in the latent space. We check if the $N$ vectors are distanced at least with a threshold to make sure that they do not belong to the same class. Our algorithm is described in detail in algorithm~\ref{alg}.





% Next, having the $N$ vectors sampled from the latent space representation, we generate another $N$ vectors by a policy $\mathcal{P}$. The goal of policy $\mathcal{P}$ is to generate vectors belonging to the same classes of the initial $N$ vectors.


%\begin{figure}
 %   \centering
 %   \includegraphics[width=0.5\linewidth]{figures/GAN/Method/latent_space_visualization.png}
  %  \includegraphics[width=0.5\linewidth]{figures/GAN/Method/latent_space_visualization2.png}
%    \caption{latent space representation visualization.}
 %   \label{fig:latent_space_visualization}
%\end{figure}


% \subsection{Generate tasks by variational auto encoders (VAE)}
% A compelling alternative that enables task construction could be using variational auto encoders. The latent space representation and decoder network in a VAE trained on our unsupervised dataset $\mathcal{U}$ can be exploited by proceeding in a similar manner as GANs. In our experiments, we evaluate the results on VAEs as well. First, we sample $N$ vectors (images) from $\mathcal{U}$ then, we input it to the \emph{Encoder Network} of the VAE to generate another $N$ vectors. Next, we perturb these samples with a Gaussian noise and input it to the \emph{Decoder Network} of the VAE whose outputs are the images for the validation. This method which we refer as LASIUM-VAE allows us to use real images of the dataset in constructing tasks. Fig~\ref{fig:method-vae} sketches the way that the tasks are built by VAE. 




% \begin{figure*}[!t]
%     \centering
%     \begin{tabular}{cc}
%           %\includegraphics[width=3.5cm,height=2.5cm]{cost.png} & 
%                 \includegraphics[width=.53\linewidth]{figures/GAN/VAE1.png}
%  & \hspace{3mm}
%           \includegraphics[width=.4\linewidth]{figures/xxx.png} \\
          
%     \end{tabular}
% \vspace{-2mm}
%     \caption{Task construction by VAE.}\label{fig:vae}
% \vspace{-1mm}
% \end{figure*}
